Inclusive jet and hadron suppression in a multistage approach

We present a new study of jet interactions in the quark-gluon plasma created in high-energy heavy-ion collisions, using a multistage event generator within the JETSCAPE framework. We focus on medium-induced modifications in the rate of inclusive jets and high transverse momentum (high-$p_{\mathrm{T}}$) hadrons. Scattering-induced jet energy loss is calculated in two stages: A high virtuality stage based on the MATTER model, in which scattering of highly virtual partons modifies the vacuum radiation pattern, and a second stage at lower jet virtuality based on the LBT model, in which leading partons gain and lose virtuality by scattering and radiation. Coherence effects that reduce the medium-induced emission rate in the MATTER phase are also included. The TRENTo model is used for initial conditions, and the (2+1)dimensional VISHNU model is used for viscous hydrodynamic evolution. Jet interactions with the medium are modeled via 2-to-2 scattering with Debye screened potentials, in which the recoiling partons are tracked, hadronized, and included in the jet clustering. Holes left in the medium are also tracked and subtracted to conserve transverse momentum. Calculations of the nuclear modification factor ($R_{\mathrm{AA}}$) for inclusive jets and high-$p_{\mathrm{T}}$ hadrons are compared to experimental measurements at the BNL Relativistic Heavy Ion Collider (RHIC) and the CERN Large Hadron Collider (LHC). Within this framework, we find that with one extra parameter which codifies the transition between stages of jet modification -- along with the typical parameters such as the coupling in the medium, the start and stop criteria etc. -- we can describe these data at all energies for central and semicentral collisions without a rescaling of the jet transport coefficient $\hat{q}$.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
